iDb-RRT: Sampling-based Kinodynamic Motion Planning with Motion Primitives and Trajectory Optimization

Rapidly-exploring Random Trees (RRT) and its variations have emerged as a robust and efficient tool for finding collision-free paths in robotic systems. However, adding dynamic constraints makes the motion planning problem significantly harder, as it requires solving two-value boundary problems (computationally expensive) or propagating random control inputs (uninformative). Alternatively, Iterative Discontinuity Bounded A* (iDb-A*), introduced in our previous study, combines search and optimization iteratively. The search step connects short trajectories (motion primitives) while allowing a bounded discontinuity between the motion primitives, which is later repaired in the trajectory optimization step. Building upon these foundations, in this paper, we present iDb-RRT, a sampling-based kinodynamic motion planning algorithm that combines motion primitives and trajectory optimization within the RRT framework. iDb-RRT is probabilistically complete and can be implemented in forward or bidirectional mode. We have tested our algorithm across a benchmark suite comprising 30 problems, spanning 8 different systems, and shown that iDb-RRT can find solutions up to 10x faster than previous methods, especially in complex scenarios that require long trajectories or involve navigating through narrow passages.

==> related.tex <==

\textbf{Search-based} approaches rely on existing methods for discrete path planning, such as A* and its variants.
The common approach is to generate short trajectories (\emph{motion primitives}) using a state lattice -- a pre-specified discrete set of states~\cite{pivtoraikoKinodynamicMotionPlanning2011, pivtoraiko2005efficient}.
Each primitive starts and ends at a grid cell, and swept cells can be precomputed for efficient collision checking.
Once motion primitives are computed, existing algorithms such as A* or an anytime variant (e.g., Anytime Repairing A* \cite{likhachev2003ara}) can be employed without modification, providing very strong theoretical guarantees on both optimality and completeness with respect to the chosen primitives.
The major challenge is selecting and computing effective motion primitives, especially for high-dimensional systems~\cite{PivtoraikoThesis, dispersionMinimizingPrimitives}.

\textbf{Sampling-based} approaches build a tree \(\mathcal{T}\) rooted at the start state \(\mathbf{x}_s\).
During tree expansion, i) a random state \(\mathbf{x}_{\text{rand}}\) in the state space is sampled, ii) an existing state \(\mathbf{x}_{\text{expand}} \in \mathcal{T}\) is selected, and iii) a new state \(\mathbf{x}_{\text{new}}\) is added with a motion that starts at \(\mathbf{x}_{\text{expand}}\) and moves towards \(\mathbf{x}_{\text{rand}}\).
In system with dynamics constraints, there are two 

The motions are typically generated by propagating random control inputs, and the classic version of this approach, \emph{kinodynamic RRT}~\cite{kinodynamicRRT}, is probabilistically complete~\cite{kunzKinodynamicRRTsFixed2015}.
Asymptotic optimality can be achieved when planning in state-cost space (\emph{AO-RRT})~\cite{AO-RRT, AO-RRT-Analysis, ST-RRT-Star} or by computing a sparse tree (\emph{SST*})~\cite{SSTstar}.
These methods rely on a distance function and often require fast nearest neighbor data structures, such as k-d trees, for efficiency.

Sampling-based approaches are designed to explore the state space as rapidly as possible and typically do not explicitly use a heuristic function, unlike search-based methods.
Instead, the exploration/exploitation trade-off is controlled by using goal-biasing.
In these approaches, the goal constraint is typically reformulated using a goal region rather than a goal state.

\textbf{Optimization-based} approaches locally refine an initial trajectory using the gradients of the cost function, dynamics, and collision constraints, unlike the previous gradient-free methods.
The trajectory optimization problem can be formulated as a finite-dimensional nonlinear program (NLP) using either direct collocation or shooting methods~\cite{betts2010practical}, and solved with general-purpose nonlinear solvers (e.g., \cite{wachter2006implementation, gill2005snopt}).

For instance, \emph{TrajOpt}~\cite{TrajOpt} and \emph{GuSTO}~\cite{GuSTO,malyutaConvexOptimizationTrajectory2021} rely on direct transcription and sequential convex programming (SCP), while \emph{KOMO}~\cite{KOMO} combines direct transcription with the Augmented Lagrangian algorithm.

Trajectories can also be computed with optimal control solvers based on Differential Dynamic Programming~\cite{Crocoddyl, howell2019altro} or the iterative Linear Quadratic Regulator (iLQR)~\cite{li2004iterative}.

All optimization-based approaches require an initial guess as a starting trajectory, but this guess does not necessarily need to be feasible.
For nonlinear dynamics and constraints, optimization approaches are incomplete and might fail or converge to a local optimum.


In fact, they often converge to infeasible solutions unless the initial guess is close to a feasible solution.
When successful, the solution quality is significantly higher (e.g., in terms of smoothness) compared to sampling-based or search-based approaches.
Moreover, optimization-based approaches do not suffer directly from the curse of dimensionality, although higher dimensions might result in more local optima.

\textbf{Hybrid} approaches combine search, sampling, and optimization.
For instance, one can combine search and optimization~\cite{natarajanInterleavingGraphSearch2021}, search and sampling~\cite{sakcakSamplingbasedOptimalKinodynamic2019, DIRT, shomeAsymptoticallyOptimalKinodynamic2021b}, or combine sampling and optimization~\cite{RABITstar, kamat2022bitkomo}.
For some dynamical systems, using insights from control theory for motion planning can also be beneficial \cite{LQR-RRTstar, kino-RRTstar, R3T}, but it requires domain knowledge.
Motion planning can also benefit from using machine learning for computational efficiency~\cite{RL-RRT, L-SBMP}.

Our algorithm, iDb-A*, combines ideas and tools from the three main approaches to kinodynamic motion planning.
The most closely related works are methods that reuse edges within a sampling-based planning framework~\cite{shomeAsymptoticallyOptimalKinodynamic2021b} and search-based methods with duplicate detection~\cite{duEscapingLocalMinima2019}.
Compared to these works, we include trajectory optimization and reuse locally optimal precomputed motion primitives interconnected with bounded discontinuity for better success and faster convergence.

Apart from the aforementioned approaches, a popular approach to kinodynamic motion planning problems is to first plan with \textbf{simplified dynamic models} and to use trajectory optimization or a local controller to follow the reference path while accounting for the true dynamics.
The simplest model is a geometric model (holonomic, first-order integrator), which enables geometric motion planning with, e.g., RRT, RRT*, PRM, or PRM* \cite{karaman2011sampling, kavraki1996probabilistic, lavalle1998rapidly}.
Second-order systems can be approximated by a double integrator linear model \cite{webb2012kinodynamic}.

The trajectories computed with simplified dynamics can then be used as initial guesses for trajectory optimization (that is, optimization-based approaches as previously discussed), model predictive control, or system-specific controllers for quadcopters \cite{lee2010geometric}, unicycle-like robots~\cite{kim2002controllers}, or car-like robots~\cite{laumond1998robot}.
System-specific motion planners can exploit certain properties of the dynamics, such as differential flatness in quadcopters, which allows faster motion planning as shown for quadcopters~\cite{mellinger2011minimum} and for some specific fixed-wing UAVs~\cite{bry2015aggressive}.
However, differential flatness cannot account for actuation constraints directly -- leading to either conservative or infeasible trajectories, especially for small UAVs with a low thrust-to-weight ratio.

Notably, planning with simplified dynamics does not guarantee the generation of valid motion plans and demands an in-depth understanding of the dynamical system.
In our algorithm, iDb-A*, connecting motion primitives with bounded discontinuity during the search step can be interpreted as an alternative form of simplified dynamics.
However, iDb-A* is complete and asymptotically optimal because it combines search and optimization in an iterative fashion, increasing the number of motion primitives and reducing the allowed discontinuity in each iteration.


==> results/by_hand_merge.tex <==
\begin{tabular}{lcccccccccccccccc}
\toprule
 Problem  &\multicolumn{4}{c}{d0r}&\multicolumn{4}{c}{d1r}&\multicolumn{4}{c}{d2r}&\multicolumn{4}{c}{idr}\\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
 &  p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c\\
\midrule
Car with trailer/Kink & 1.00 & 0.26 & 0.06 & 51.25 & 1.00 & { \color{cyan} 0.24} & { \color{cyan} 0.02} & { \color{red} 61.05} & 1.00 & 0.29 & 0.04 & 56.55 & 1.00 & { \color{red} 1.42} & { \color{red} 1.23} & { \color{cyan} 31.10}\\
Car with trailer/Park & 1.00 & 0.09 & { \color{cyan} 0.01} & { \color{cyan} 10.25} & 1.00 & { \color{cyan} 0.07} & { \color{cyan} 0.00} & 10.55 & 1.00 & { \color{red} 0.10} & { \color{cyan} 0.00} & 13.05 & 1.00 & { \color{red} 0.11} & { \color{cyan} 0.01} & { \color{red} 17.00}\\
Planar rotor/Hole & 1.00 & 1.16 & 0.88 & 10.32 & 1.00 & 1.01 & 0.61 & 10.03 & 1.00 & { \color{cyan} 0.70} & { \color{cyan} 0.35} & { \color{red} 11.03} & 0.90 & { \color{red} 13.68} & { \color{red} 13.11} & { \color{cyan} 3.46}\\
Planar rotor/Bugtrap & 1.00 & 1.08 & 0.57 & { \color{red} 9.73} & 1.00 & { \color{cyan} 0.54} & { \color{cyan} 0.11} & 9.13 & 1.00 & 0.85 & 0.27 & 9.41 & 1.00 & { \color{red} 12.02} & { \color{red} 11.44} & { \color{cyan} 5.17}\\
Rotor pole/Swing up obstacles & 1.00 & { \color{red} 6.44} & { \color{red} 5.67} & 8.42 & 1.00 & { \color{cyan} 0.86} & { \color{cyan} 0.16} & 7.85 & 1.00 & 1.18 & 0.22 & { \color{red} 8.52} & 1.00 & 3.25 & 2.84 & { \color{cyan} 3.98}\\
Rotor pole/Small window & 1.00 & 4.53 & 3.78 & { \color{red} 10.96} & 1.00 & { \color{cyan} 1.07} & { \color{cyan} 0.14} & 9.41 & 1.00 & 1.52 & 0.30 & 7.88 & 1.00 & { \color{red} 4.79} & { \color{red} 4.48} & { \color{cyan} 4.54}\\
Quadrotor v0/Recovery & 1.00 & { \color{cyan} 0.66} & 0.20 & 5.42 & 1.00 & 0.99 & { \color{red} 0.36} & { \color{red} 5.59} & 1.00 & { \color{cyan} 0.65} & 0.15 & { \color{cyan} 5.12} & 1.00 & { \color{red} 1.44} & { \color{cyan} 0.03} & 5.56\\
Quadrotor v0/Recovery obstacles & 1.00 & { \color{red} 1.78} & 0.46 & 6.87 & 1.00 & { \color{red} 1.78} & { \color{red} 0.83} & 6.86 & 1.00 & { \color{cyan} 1.59} & 0.38 & { \color{red} 7.49} & 1.00 & 1.64 & { \color{cyan} 0.23} & { \color{cyan} 5.74}\\
Quadrotor v1/Obstacle & 1.00 & { \color{cyan} 0.70} & { \color{cyan} 0.15} & 5.16 & 1.00 & 1.17 & 0.39 & 8.32 & 1.00 & 1.19 & 0.47 & { \color{red} 8.47} & 1.00 & { \color{red} 2.76} & { \color{red} 1.00} & { \color{cyan} 4.54}\\
Quadrotor v1/Window & 1.00 & { \color{cyan} 0.66} & { \color{cyan} 0.24} & 5.48 & 1.00 & 0.75 & 0.26 & 5.44 & 1.00 & 0.95 & 0.34 & { \color{red} 5.72} & 1.00 & { \color{red} 1.85} & { \color{red} 0.37} & { \color{cyan} 3.70}\\
Unicycle 1 v0/Bugtrap & 1.00 & 0.14 & 0.04 & 32.60 & 1.00 & 0.15 & { \color{cyan} 0.01} & 32.80 & 1.00 & { \color{cyan} 0.11} & { \color{cyan} 0.01} & { \color{red} 33.95} & 1.00 & { \color{red} 0.55} & { \color{red} 0.49} & { \color{cyan} 22.20}\\
Unicycle 1 v2/Wall & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -}\\
Unicycle 2/Bugtrap & 1.00 & 0.19 & 0.09 & { \color{red} 58.60} & 1.00 & { \color{cyan} 0.08} & { \color{cyan} 0.01} & 56.55 & 1.00 & 0.10 & { \color{cyan} 0.02} & 54.60 & 1.00 & { \color{red} 1.70} & { \color{red} 1.59} & { \color{cyan} 25.30}\\
Unicycle 2/Park & 1.00 & { \color{cyan} 0.02} & { \color{cyan} 0.01} & 10.40 & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & { \color{red} 12.55} & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & 10.80 & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & { \color{cyan} 5.80}\\
\midrule
Car with trailer/bugtrap\_double & 1.00 & 0.73 & 0.24 & { \color{red} 101.60} & 1.00 & { \color{cyan} 0.67} & 0.18 & 96.80 & 1.00 & 0.70 & { \color{cyan} 0.17} & 100.15 & 1.00 & { \color{red} 1.69} & { \color{red} 1.13} & { \color{cyan} 46.80}\\
Car with trailer/narrow\_passage & 1.00 & 0.64 & 0.18 & 123.00 & 1.00 & 0.67 & { \color{cyan} 0.11} & { \color{red} 131.15} & 1.00 & { \color{cyan} 0.59} & 0.12 & 127.50 & 1.00 & { \color{red} 8.74} & { \color{red} 8.42} & { \color{cyan} 53.90}\\
Planar rotor/narrow\_passage & 1.00 & 2.34 & 0.64 & { \color{cyan} 16.16} & 1.00 & { \color{cyan} 1.76} & 0.39 & 17.52 & 1.00 & 1.83 & { \color{cyan} 0.33} & 17.51 & 0.00 & { \color{red} inf} & { \color{red} inf} & { \color{red} inf}\\
Planar rotor/Recovery obstacles\_double & 1.00 & { \color{cyan} 0.44} & 0.13 & 9.29 & 1.00 & 0.62 & { \color{cyan} 0.09} & 11.09 & 1.00 & 0.48 & { \color{cyan} 0.09} & { \color{red} 11.17} & 1.00 & { \color{red} 17.08} & { \color{red} 16.33} & { \color{cyan} 6.03}\\
Planar rotor/Bugtrap\_double & 1.00 & 1.90 & 0.50 & 13.08 & 1.00 & { \color{cyan} 1.64} & { \color{cyan} 0.25} & { \color{cyan} 12.59} & 1.00 & 1.68 & 0.31 & 12.66 & 0.00 & { \color{red} inf} & { \color{red} inf} & { \color{red} inf}\\
Rotor pole/Swing up obstacles2 & 1.00 & 12.73 & 10.74 & { \color{red} 12.95} & 1.00 & { \color{cyan} 1.66} & { \color{cyan} 0.13} & 11.21 & 1.00 & 2.11 & 0.36 & 12.06 & 1.00 & { \color{red} 14.94} & { \color{red} 14.54} & { \color{cyan} 5.00}\\
Rotor pole/Small window2 & 1.00 & 2.65 & 1.74 & 12.48 & 1.00 & 2.59 & { \color{cyan} 0.28} & 12.30 & 1.00 & { \color{cyan} 2.12} & { \color{cyan} 0.28} & { \color{red} 12.72} & 1.00 & { \color{red} 11.97} & { \color{red} 11.50} & { \color{cyan} 6.18}\\
Quadrotor v0/bugtrap3 & 1.00 & 8.00 & 3.47 & 11.79 & 1.00 & { \color{cyan} 4.68} & { \color{cyan} 1.83} & { \color{red} 12.54} & 1.00 & 4.90 & 1.86 & 12.15 & 1.00 & { \color{red} 23.62} & { \color{red} 20.45} & { \color{cyan} 6.36}\\
Quadrotor v0/Recovery obstacles3 & 1.00 & { \color{cyan} 1.42} & 0.57 & 6.73 & 1.00 & 2.40 & 1.21 & { \color{red} 9.36} & 1.00 & 1.60 & { \color{cyan} 0.40} & 6.93 & 1.00 & { \color{red} 4.21} & { \color{red} 1.63} & { \color{cyan} 6.33}\\
Quadrotor v0/Recovery obstacles4 & 1.00 & { \color{cyan} 2.62} & { \color{cyan} 0.75} & 10.21 & 1.00 & 4.00 & 1.39 & { \color{red} 12.44} & 1.00 & 2.64 & 1.01 & 9.07 & 1.00 & { \color{red} 6.40} & { \color{red} 3.96} & { \color{cyan} 6.42}\\
Quadrotor v0/Window\_double & 1.00 & 6.24 & 2.98 & 11.34 & 1.00 & { \color{cyan} 4.26} & { \color{cyan} 1.93} & 12.04 & 1.00 & 4.91 & 1.96 & { \color{red} 13.07} & 1.00 & { \color{red} 8.28} & { \color{red} 4.45} & { \color{cyan} 6.17}\\
Quadrotor v1/bugtrap3 & 1.00 & 2.96 & 1.37 & 9.98 & 1.00 & { \color{cyan} 2.52} & { \color{cyan} 0.87} & 10.57 & 1.00 & 3.25 & 0.92 & { \color{red} 10.88} & 1.00 & { \color{red} 53.33} & { \color{red} 51.01} & { \color{cyan} 5.35}\\
Quadrotor v1/Recovery obstacles4 & 1.00 & 2.39 & 0.48 & 9.75 & 1.00 & 3.70 & { \color{cyan} 0.38} & { \color{red} 9.79} & 1.00 & { \color{cyan} 2.09} & 0.55 & 9.42 & 1.00 & { \color{red} 61.22} & { \color{red} 57.26} & { \color{cyan} 6.23}\\
Quadrotor v1/Window\_double2 & 1.00 & { \color{cyan} 1.71} & 0.77 & 8.06 & 1.00 & 2.51 & 0.82 & { \color{red} 10.67} & 1.00 & 1.88 & { \color{cyan} 0.62} & 9.71 & 1.00 & { \color{red} 25.63} & { \color{red} 22.48} & { \color{cyan} 5.10}\\
Unicycle 1 v0/bugtrap\_double & 1.00 & 0.22 & 0.08 & 60.20 & 1.00 & { \color{cyan} 0.19} & { \color{cyan} 0.04} & { \color{red} 71.45} & 1.00 & 0.20 & 0.06 & 57.30 & 1.00 & { \color{red} 0.89} & { \color{red} 0.75} & { \color{cyan} 30.10}\\
Unicycle 1 v0/narrow\_passage & 1.00 & { \color{cyan} 0.20} & 0.04 & 80.80 & 1.00 & { \color{cyan} 0.20} & { \color{cyan} 0.02} & { \color{red} 89.70} & 1.00 & { \color{cyan} 0.19} & 0.03 & 79.70 & 1.00 & { \color{red} 1.78} & { \color{red} 1.69} & { \color{cyan} 37.30}\\
Unicycle 2/bugtrap\_double & 1.00 & 0.42 & 0.17 & 86.55 & 1.00 & 0.35 & 0.15 & { \color{red} 98.45} & 1.00 & { \color{cyan} 0.31} & { \color{cyan} 0.12} & 96.10 & 1.00 & { \color{red} 2.31} & { \color{red} 2.16} & { \color{cyan} 34.60}\\
Unicycle 2/narrow\_passage & 1.00 & 0.30 & 0.11 & 121.75 & 1.00 & 0.28 & { \color{cyan} 0.06} & { \color{red} 125.05} & 1.00 & { \color{cyan} 0.23} & { \color{cyan} 0.07} & 109.45 & 1.00 & { \color{red} 7.45} & { \color{red} 7.24} & { \color{cyan} 42.70}\\
\bottomrule


\bottomrule
\end{tabular}


==> results/hand_merge_28.tex <==
\begin{tabular}{lcccccccccc}
\toprule
 Problem  &\multicolumn{2}{c}{iDb-RRT-F}&\multicolumn{2}{c}{iDb-RRT-C}&\multicolumn{2}{c}{Geo-RRT-TO}&\multicolumn{2}{c}{iDb-A*}&\multicolumn{2}{c}{Kino-RRT}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
 &  t [s] & c & t [s] & c & t [s] & c & t [s] & c & t [s] & c\\
\midrule
\midrule
Car with trailer/Kink & 0.28 & 62.05 & 0.27 & 52.45 & 0.46 & { \bf 27.50} & {  1.28} & 31.10 & { \bf 0.21} & {  68.35}\\
Car with trailer/Park & 0.15 & {  17.90} & 0.07 & 11.95 & 0.07 & { \bf 4.90} & 0.11 & {  17.90} & { \bf 0.03} & 7.55\\
Planar rotor/Hole & 0.56 & 8.41 & 0.79 & 9.87 & { \bf 0.27} & { \bf 2.83} & 10.01 & 3.40 & - & -\\
Planar rotor/Bugtrap & 1.75 & 8.27 & { \bf 0.87} & 10.71 & - & - & 15.56 & { \bf 5.16} & - & -\\
Rotor pole/Swing up obstacles & 1.96 & 8.44 & 0.95 & 8.52 & { \bf 0.50} & { \bf 3.25} & 2.97 & 3.98 & - & -\\
Rotor pole/Small window & 2.86 & 10.87 & 0.95 & 8.99 & { \bf 0.46} & { \bf 3.60} & 4.47 & 4.54 & - & -\\
Quadrotor v0/Recovery & { \bf 0.67} & { \bf 4.77} & 0.95 & 5.44 & - & - & 1.34 & 5.56 & - & -\\
Quadrotor v0/Recovery obstacles & { \bf 1.11} & 6.75 & 1.92 & 6.75 & - & - & 1.43 & { \bf 5.72} & - & -\\
Quadrotor v1/Obstacle & 0.77 & 5.40 & 1.14 & 6.85 & { \bf 0.29} & { \bf 2.57} & 2.57 & 4.53 & - & -\\
Quadrotor v1/Window & { \bf 0.87} & 6.34 & 1.00 & 5.79 & 1.00 & { \bf 2.43} & 1.68 & 3.70 & - & -\\
Unicycle 1 v0/Bugtrap & { \bf 0.12} & 36.00 & { \bf 0.12} & 36.10 & 0.27 & 29.45 & {  0.54} & { \bf 22.20} & 0.14 & 70.00\\
Unicycle 1 v2/Wall & 0.10 & 32.25 & { \bf 0.03} & 32.20 & 0.47 & 20.40 & {  0.95} & { \bf 19.60} & 0.18 & 48.85\\
Unicycle 2/Bugtrap & 0.22 & 67.15 & { \bf 0.09} & 57.60 & 0.31 & 34.30 & {  1.66} & { \bf 25.30} & 0.25 & 66.80\\
Unicycle 2/Park & 0.02 & 8.55 & { \bf 0.01} & 12.80 & {  0.07} & { \bf 5.80} & { \bf 0.01} & { \bf 5.80} & 0.03 & {  18.70}\\
\midrule
Car with trailer/bugtrap\_double & 0.69 & 85.10 & { \bf 0.58} & 97.95 & - & - & 1.76 & { \bf 46.80} & 1.18 & 101.10\\
Car with trailer/narrow\_passage & 0.63 & 119.25 & { \bf 0.60} & 127.95 & - & - & 9.06 & { \bf 53.90} & 2.31 & 139.55\\
Planar rotor/narrow\_passage & 2.20 & 15.30 & { \bf 1.49} & { \bf 14.55} & - & - & - & - & 56.63 & 22.07\\
Planar rotor/Recovery obstacles\_double & { \bf 0.51} & 10.21 & 0.61 & 11.11 & - & - & 19.26 & { \bf 6.03} & - & -\\
Planar rotor/Bugtrap\_double & 2.63 & 14.31 & { \bf 1.40} & 12.74 & - & - & - & - & - & -\\
Rotor pole/Swing up obstacles2 & 4.89 & 10.11 & { \bf 2.10} & 12.57 & 2.23 & { \bf 4.94} & 15.36 & 5.00 & - & -\\
Rotor pole/Small window2 & 4.64 & 11.89 & 1.87 & 11.96 & { \bf 0.97} & { \bf 4.48} & 12.24 & 6.18 & - & -\\
Quadrotor v0/bugtrap3 & 4.67 & 11.32 & { \bf 3.69} & 12.62 & - & - & 23.67 & { \bf 6.36} & - & -\\
Quadrotor v0/Recovery obstacles3 & 1.94 & 6.05 & 1.62 & 6.86 & { \bf 0.69} & { \bf 2.56} & 4.48 & 6.38 & - & -\\
Quadrotor v0/Recovery obstacles4 & 3.60 & 12.48 & 3.95 & 8.65 & { \bf 1.03} & { \bf 4.44} & 6.52 & 6.42 & - & -\\
Quadrotor v0/Window\_double & 6.29 & 11.04 & 4.52 & 12.76 & { \bf 3.24} & { \bf 3.17} & 8.06 & 6.08 & - & -\\
Quadrotor v1/bugtrap3 & { \bf 3.02} & 10.39 & 3.39 & 13.56 & - & - & 53.49 & { \bf 5.33} & - & -\\
Quadrotor v1/Recovery obstacles4 & 1.86 & 9.27 & 1.68 & 9.92 & { \bf 1.31} & { \bf 3.88} & 61.50 & 6.22 & - & -\\
Quadrotor v1/Window\_double2 & 2.74 & 8.71 & { \bf 2.35} & 10.53 & - & - & 26.05 & { \bf 5.08} & - & -\\
Unicycle 1 v0/bugtrap\_double & 0.23 & 59.00 & 0.22 & 64.95 & 0.87 & 42.95 & {  0.94} & { \bf 30.10} & 0.22 & {  103.55}\\
Unicycle 1 v0/narrow\_passage & 0.18 & 87.55 & 0.21 & 90.85 & 0.62 & 50.70 & {  1.92} & { \bf 37.30} & { \bf 0.16} & {  136.70}\\
Unicycle 2/bugtrap\_double & { \bf 0.31} & 92.00 & 0.40 & 93.15 & 0.54 & 54.50 & {  2.44} & { \bf 34.60} & 0.34 & {  114.50}\\
Unicycle 2/narrow\_passage & 0.32 & 110.90 & { \bf 0.21} & 119.00 & 0.38 & 58.20 & {  7.64} & { \bf 42.70} & 0.30 & 135.05\\



\bottomrule
\end{tabular}


==> results/summary_iros_2024-02-26--13-47-01.tex <==
\begin{tabular}{lcccccccccccccccc}
\toprule
 Problem  &\multicolumn{4}{c}{d0r}&\multicolumn{4}{c}{d1r}&\multicolumn{4}{c}{d2r}&\multicolumn{4}{c}{idr}\\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
 &  p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c\\
\midrule
Car with trailer/Kink & 1.00 & 0.26 & 0.06 & 51.25 & 1.00 & { \color{cyan} 0.24} & { \color{cyan} 0.02} & { \color{red} 61.05} & 1.00 & 0.29 & 0.04 & 56.55 & 1.00 & { \color{red} 1.42} & { \color{red} 1.23} & { \color{cyan} 31.10}\\
Car with trailer/Park & 1.00 & 0.09 & { \color{cyan} 0.01} & { \color{cyan} 10.25} & 1.00 & { \color{cyan} 0.07} & { \color{cyan} 0.00} & 10.55 & 1.00 & { \color{red} 0.10} & { \color{cyan} 0.00} & 13.05 & 1.00 & { \color{red} 0.11} & { \color{cyan} 0.01} & { \color{red} 17.00}\\
Planar rotor/Hole & 1.00 & 1.16 & 0.88 & 10.32 & 1.00 & 1.01 & 0.61 & 10.03 & 1.00 & { \color{cyan} 0.70} & { \color{cyan} 0.35} & { \color{red} 11.03} & 0.90 & { \color{red} 13.68} & { \color{red} 13.11} & { \color{cyan} 3.46}\\
Planar rotor/Bugtrap & 1.00 & 1.08 & 0.57 & { \color{red} 9.73} & 1.00 & { \color{cyan} 0.54} & { \color{cyan} 0.11} & 9.13 & 1.00 & 0.85 & 0.27 & 9.41 & 1.00 & { \color{red} 12.02} & { \color{red} 11.44} & { \color{cyan} 5.17}\\
Rotor pole/Swing up obstacles & 1.00 & { \color{red} 6.44} & { \color{red} 5.67} & 8.42 & 1.00 & { \color{cyan} 0.86} & { \color{cyan} 0.16} & 7.85 & 1.00 & 1.18 & 0.22 & { \color{red} 8.52} & 1.00 & 3.25 & 2.84 & { \color{cyan} 3.98}\\
Rotor pole/Small window & 1.00 & 4.53 & 3.78 & { \color{red} 10.96} & 1.00 & { \color{cyan} 1.07} & { \color{cyan} 0.14} & 9.41 & 1.00 & 1.52 & 0.30 & 7.88 & 1.00 & { \color{red} 4.79} & { \color{red} 4.48} & { \color{cyan} 4.54}\\
Quadrotor v0/Recovery & 1.00 & { \color{cyan} 0.66} & 0.20 & 5.42 & 1.00 & 0.99 & { \color{red} 0.36} & { \color{red} 5.59} & 1.00 & { \color{cyan} 0.65} & 0.15 & { \color{cyan} 5.12} & 1.00 & { \color{red} 1.44} & { \color{cyan} 0.03} & 5.56\\
Quadrotor v0/Recovery obstacles & 1.00 & { \color{red} 1.78} & 0.46 & 6.87 & 1.00 & { \color{red} 1.78} & { \color{red} 0.83} & 6.86 & 1.00 & { \color{cyan} 1.59} & 0.38 & { \color{red} 7.49} & 1.00 & 1.64 & { \color{cyan} 0.23} & { \color{cyan} 5.74}\\
Quadrotor v1/Obstacle & 1.00 & { \color{cyan} 0.70} & { \color{cyan} 0.15} & 5.16 & 1.00 & 1.17 & 0.39 & 8.32 & 1.00 & 1.19 & 0.47 & { \color{red} 8.47} & 1.00 & { \color{red} 2.76} & { \color{red} 1.00} & { \color{cyan} 4.54}\\
Quadrotor v1/Window & 1.00 & { \color{cyan} 0.66} & { \color{cyan} 0.24} & 5.48 & 1.00 & 0.75 & 0.26 & 5.44 & 1.00 & 0.95 & 0.34 & { \color{red} 5.72} & 1.00 & { \color{red} 1.85} & { \color{red} 0.37} & { \color{cyan} 3.70}\\
Unicycle 1 v0/Bugtrap & 1.00 & 0.14 & 0.04 & 32.60 & 1.00 & 0.15 & { \color{cyan} 0.01} & 32.80 & 1.00 & { \color{cyan} 0.11} & { \color{cyan} 0.01} & { \color{red} 33.95} & 1.00 & { \color{red} 0.55} & { \color{red} 0.49} & { \color{cyan} 22.20}\\
Unicycle 1 v2/Wall & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -} & - & { \color{cyan} -} & { \color{cyan} -} & { \color{cyan} -}\\
Unicycle 2/Bugtrap & 1.00 & 0.19 & 0.09 & { \color{red} 58.60} & 1.00 & { \color{cyan} 0.08} & { \color{cyan} 0.01} & 56.55 & 1.00 & 0.10 & { \color{cyan} 0.02} & 54.60 & 1.00 & { \color{red} 1.70} & { \color{red} 1.59} & { \color{cyan} 25.30}\\
Unicycle 2/Park & 1.00 & { \color{cyan} 0.02} & { \color{cyan} 0.01} & 10.40 & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & { \color{red} 12.55} & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & 10.80 & 1.00 & { \color{cyan} 0.01} & { \color{cyan} 0.00} & { \color{cyan} 5.80}\\
\bottomrule
\end{tabular}


==> results/summary_iros_2024-02-26--14-22-04.tex <==
\begin{tabular}{lcccccccccccccccc}
\toprule
 Problem  &\multicolumn{4}{c}{d0r}&\multicolumn{4}{c}{d1r}&\multicolumn{4}{c}{d2r}&\multicolumn{4}{c}{idr}\\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
 &  p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c & p & t [s] & t\_raw [s] & c\\
\midrule
Car with trailer/bugtrap\_double & 1.00 & 0.73 & 0.24 & { \color{red} 101.60} & 1.00 & { \color{cyan} 0.67} & 0.18 & 96.80 & 1.00 & 0.70 & { \color{cyan} 0.17} & 100.15 & 1.00 & { \color{red} 1.69} & { \color{red} 1.13} & { \color{cyan} 46.80}\\
Car with trailer/narrow\_passage & 1.00 & 0.64 & 0.18 & 123.00 & 1.00 & 0.67 & { \color{cyan} 0.11} & { \color{red} 131.15} & 1.00 & { \color{cyan} 0.59} & 0.12 & 127.50 & 1.00 & { \color{red} 8.74} & { \color{red} 8.42} & { \color{cyan} 53.90}\\
Planar rotor/narrow\_passage & 1.00 & 2.34 & 0.64 & { \color{cyan} 16.16} & 1.00 & { \color{cyan} 1.76} & 0.39 & 17.52 & 1.00 & 1.83 & { \color{cyan} 0.33} & 17.51 & 0.00 & { \color{red} inf} & { \color{red} inf} & { \color{red} inf}\\
Planar rotor/Recovery obstacles\_double & 1.00 & { \color{cyan} 0.44} & 0.13 & 9.29 & 1.00 & 0.62 & { \color{cyan} 0.09} & 11.09 & 1.00 & 0.48 & { \color{cyan} 0.09} & { \color{red} 11.17} & 1.00 & { \color{red} 17.08} & { \color{red} 16.33} & { \color{cyan} 6.03}\\
Planar rotor/Bugtrap\_double & 1.00 & 1.90 & 0.50 & 13.08 & 1.00 & { \color{cyan} 1.64} & { \color{cyan} 0.25} & { \color{cyan} 12.59} & 1.00 & 1.68 & 0.31 & 12.66 & 0.00 & { \color{red} inf} & { \color{red} inf} & { \color{red} inf}\\
Rotor pole/Swing up obstacles2 & 1.00 & 12.73 & 10.74 & { \color{red} 12.95} & 1.00 & { \color{cyan} 1.66} & { \color{cyan} 0.13} & 11.21 & 1.00 & 2.11 & 0.36 & 12.06 & 1.00 & { \color{red} 14.94} & { \color{red} 14.54} & { \color{cyan} 5.00}\\
Rotor pole/Small window2 & 1.00 & 2.65 & 1.74 & 12.48 & 1.00 & 2.59 & { \color{cyan} 0.28} & 12.30 & 1.00 & { \color{cyan} 2.12} & { \color{cyan} 0.28} & { \color{red} 12.72} & 1.00 & { \color{red} 11.97} & { \color{red} 11.50} & { \color{cyan} 6.18}\\
Quadrotor v0/bugtrap3 & 1.00 & 8.00 & 3.47 & 11.79 & 1.00 & { \color{cyan} 4.68} & { \color{cyan} 1.83} & { \color{red} 12.54} & 1.00 & 4.90 & 1.86 & 12.15 & 1.00 & { \color{red} 23.62} & { \color{red} 20.45} & { \color{cyan} 6.36}\\
Quadrotor v0/Recovery obstacles3 & 1.00 & { \color{cyan} 1.42} & 0.57 & 6.73 & 1.00 & 2.40 & 1.21 & { \color{red} 9.36} & 1.00 & 1.60 & { \color{cyan} 0.40} & 6.93 & 1.00 & { \color{red} 4.21} & { \color{red} 1.63} & { \color{cyan} 6.33}\\
Quadrotor v0/Recovery obstacles4 & 1.00 & { \color{cyan} 2.62} & { \color{cyan} 0.75} & 10.21 & 1.00 & 4.00 & 1.39 & { \color{red} 12.44} & 1.00 & 2.64 & 1.01 & 9.07 & 1.00 & { \color{red} 6.40} & { \color{red} 3.96} & { \color{cyan} 6.42}\\
Quadrotor v0/Window\_double & 1.00 & 6.24 & 2.98 & 11.34 & 1.00 & { \color{cyan} 4.26} & { \color{cyan} 1.93} & 12.04 & 1.00 & 4.91 & 1.96 & { \color{red} 13.07} & 1.00 & { \color{red} 8.28} & { \color{red} 4.45} & { \color{cyan} 6.17}\\
Quadrotor v1/bugtrap3 & 1.00 & 2.96 & 1.37 & 9.98 & 1.00 & { \color{cyan} 2.52} & { \color{cyan} 0.87} & 10.57 & 1.00 & 3.25 & 0.92 & { \color{red} 10.88} & 1.00 & { \color{red} 53.33} & { \color{red} 51.01} & { \color{cyan} 5.35}\\
Quadrotor v1/Recovery obstacles4 & 1.00 & 2.39 & 0.48 & 9.75 & 1.00 & 3.70 & { \color{cyan} 0.38} & { \color{red} 9.79} & 1.00 & { \color{cyan} 2.09} & 0.55 & 9.42 & 1.00 & { \color{red} 61.22} & { \color{red} 57.26} & { \color{cyan} 6.23}\\
Quadrotor v1/Window\_double2 & 1.00 & { \color{cyan} 1.71} & 0.77 & 8.06 & 1.00 & 2.51 & 0.82 & { \color{red} 10.67} & 1.00 & 1.88 & { \color{cyan} 0.62} & 9.71 & 1.00 & { \color{red} 25.63} & { \color{red} 22.48} & { \color{cyan} 5.10}\\
Unicycle 1 v0/bugtrap\_double & 1.00 & 0.22 & 0.08 & 60.20 & 1.00 & { \color{cyan} 0.19} & { \color{cyan} 0.04} & { \color{red} 71.45} & 1.00 & 0.20 & 0.06 & 57.30 & 1.00 & { \color{red} 0.89} & { \color{red} 0.75} & { \color{cyan} 30.10}\\
Unicycle 1 v0/narrow\_passage & 1.00 & { \color{cyan} 0.20} & 0.04 & 80.80 & 1.00 & { \color{cyan} 0.20} & { \color{cyan} 0.02} & { \color{red} 89.70} & 1.00 & { \color{cyan} 0.19} & 0.03 & 79.70 & 1.00 & { \color{red} 1.78} & { \color{red} 1.69} & { \color{cyan} 37.30}\\
Unicycle 2/bugtrap\_double & 1.00 & 0.42 & 0.17 & 86.55 & 1.00 & 0.35 & 0.15 & { \color{red} 98.45} & 1.00 & { \color{cyan} 0.31} & { \color{cyan} 0.12} & 96.10 & 1.00 & { \color{red} 2.31} & { \color{red} 2.16} & { \color{cyan} 34.60}\\
Unicycle 2/narrow\_passage & 1.00 & 0.30 & 0.11 & 121.75 & 1.00 & 0.28 & { \color{cyan} 0.06} & { \color{red} 125.05} & 1.00 & { \color{cyan} 0.23} & { \color{cyan} 0.07} & 109.45 & 1.00 & { \color{red} 7.45} & { \color{red} 7.24} & { \color{cyan} 42.70}\\
\bottomrule
\end{tabular}

